Estimating animal utilization distributions from multiple data types: a joint spatio-temporal point process framework

Models of the spatial distribution of animals provide useful tools to help ecologists quantify species-environment relationships, and they are increasingly being used to help determine the impacts of climate and habitat changes on species. While high-quality survey-style data with known effort are sometimes available, often researchers have multiple datasets of varying quality and type. In particular, collections of sightings made by citizen scientists are becoming increasingly common, with no information typically provided on their observer effort. Many standard modelling approaches ignore observer effort completely, which can severely bias estimates of an animal's distribution. Combining sightings data from observers who followed different protocols is challenging. Any differences in observer skill, spatial effort, and the detectability of the animals across space all need to be accounted for. To achieve this, we build upon the recent advancements made in integrative species distribution models and present a novel marked spatio-temporal point process framework for estimating the utilization distribution (UD) of the individuals of a highly mobile species. We show that in certain settings, we can also use the framework to combine the UDs from the sampled individuals to estimate the species' distribution. We combine the empirical results from a simulation study with the implications outlined in a causal directed acyclic graph to identify the necessary assumptions required for our framework to control for observer effort when it is unknown. We then apply our framework to combine multiple datasets collected on the endangered Southern Resident Killer Whales, to estimate their monthly effort-corrected space-use.

==> Graveyard.tex <==

%Accurate knowledge of species' population density is vital for ecologists to develop and implement successful and targeted management and conservation policies to determine the impacts of future climate and habitat changes on species. For mobile species, gold-standard survey sampling methods, including the two popular methods: capture-recapture (CR) and distance sampling (DS; cite list of references), turn to design-based statistics to estimate the probability of detection for each individual. Both methods involve the sampling of a subset of the area of interest, and hence Horwitz-Thompson style inverse-weighting can then be used to account for un-detected individuals to estimate total population size. Crucially, it is the random placement of samplers (i.e. random choice of positions to sample), independent from the underlying species' density, that enables the Horwitz-Thompson style adjustments to be valid. \\

%Recent work has attempted to place such datasets under model-based frameworks (cite Blue whale paper and Unifying model.. Borchers et al) to allow for the estimation of the spatial distribution of the species and to investigate species-covariate associations. Interestingly, almost all approaches have considered the true species' density as coming from a spatial point process, either in the form of a inhomogeneous Poisson process (IPP hereafter) or a log-Gaussian Cox process (LGCP hereafter). To account for the partial realisation due to incomplete sampling, for example along planned survey lines or at capture sites, distance-based detection probability surfaces are used to thin the underlying species' spatial point process intensity. Thus a multiplicative decomposition of the observed intensity surface into a true intensity surface surface and a detection probability surface is assumed. It is this thinned spatial point process that is now assumed to be the observed data generating mechanism. The half-norm function is one example of a commonly used detection probability surface used to thin the true underlying intensity. \\ 


%Unfortunately, whilst survey sampling is the gold standard, such datasets are by no means the standard dataset available for ecologists looking to estimate a mobile species' spatial distribution. `Citizen science' opportunistic sightings databases are commonplace, and typically lack knowledge of observer effort. These presence-only databases typically suffer from spatially-inhomogeneous observer effort, and to make matters worse, this effort is often focused in areas of highest species' intensity. This is often referred to as preferential sampling (cite Diggle and me). Furthermore, such databases often suffer from spatially-varying species and/or individual misclassification rates, spatially-varying reporting probabilities and many other flaws. Of crucial importance to our later analysis, individual sightings within opportunistic sightings databases may not be independent of one another. This may be due to the same observer `following' an animal and reporting their repeated sightings to the database (i.e. autocorrelated sightings), or may be due to observers sharing knowledge of the species' locations between each other (i.e. a lack of independence between observers).\\ 

%Despite these efforts to adapt the logistic regression and MaxEnt models, they remain non scale-invariant. Consequently, combining data sources of differing type is not straightforward.   %As \citet{fithian2015bias} pointed out, the method ``does not distinguish between inaccessible regions and regions in which all the species are not very prevalent." \\ 

%Since then, additional methods have been proposed to extend logistic regression and MaxEnt methods to account for false negatives \citep{nichols2008multi} and false positives \citep{miller2011improving, hanks2011reconciling}, as well as to account for correlations between sighting events between different observers at the same site \citep{clare2017pairing}. Additionally, the joint modeling of multiple species by sharing model terms across the species' models was introduced by  \citet{elith2007predicting} with the aim of improving predictive performance by borrowing strength. Despite these efforts to adapt the logistic regression and MaxEnt models, they remain non scale-invariant. Consequently, combining data sources of differing type is not straightforward. 

 These typically assume that individuals have unique home range centers to be estimated, and move relative to their home range centers according to a UD. These are often assumed to take a simplified form such as a bivariate normal density centered at the estimated home range center \citep{royle2011spatial}. The parameters of these UD's are then estimated. Given the UD of every individual of a population, the spatio-temporal distribution of the population can then be calculated as a suitable combination of the individuals' UD's. These methods have also been adapted for the setting where sightings are made by mobile observers (e.g.\ vehicular-based) instead of static observers (e.g.\ camera traps) \citep{royle2011spatial}. However, the simplified form assumed of the UD in spatial capture recapture methods is undesirable in many settings, including our own. To allow for arbitrarily complex UDs to be modeled, we turn to point process methodologies. 
Multiple datasets that differ in type (e.g.\ presence-absence, presence-only, etc.,) and in data-collection protocol (distance sampling, opportunistic, etc.,) are often available.


%Furthermore, they assumed that individuals could not be uniquely identified. Thus, how to adapt their approach to estimate These conditions render current point process models unsuitable for modeling datasets with individually-identified sightings of a highly mobile species, with sightings made from a group of opportunistic observers moving continuously through space. This is because the definition of the intensity surface defining the point process models is ill-defined. To adapt the point process framework for use with a collection of sightings of an individual, we redefine the definition of the intensity surface being modeled as an encounter rate. This allows us to relax the assumptions above and present an integrative framework for estimating the spatio-temporal distribution of a mobile species that allows to merge data types with different biases in search effort and provide more precise estimates.

%Inhomogeneous Poisson process models assume the sighting locations are independent conditional upon the intensity. However, sightings of highly mobile species may remain severely autocorrelated after conditioning on the intensity if reported sightings of the same individuals occur at a high frequency relative to their movement. If we assume that the individual's movement process is with respect to a stationary invariant density (i.e.\ their UD), then enough time must be allowed between sightings to let the individuals mix with respect to their UD. This may require data to be manually subsetted accordingly to ensure approximate independence between sightings. A failure to do this, risks biasing estimates of the species' distribution \citep{johnson2013estimating, mcdonald2013point}. Furthermore, spatio-temporal correlations may also exist due to unmeasured spatially-smooth covariates and/or biological processes driving the true intensity of the target species \citep{pacifici2017integrating, yuan2017point}. Extending the thinned IPP framework to the log-Gaussian Cox process framework can help adjust for such autocorrelations \citep{chakraborty2011point}.

%This problem is faced in this paper, however to address it, we instead manually subset sightings to ensure the conditional assumption approach is satisfied. We discuss this approach in detail to assist researchers in future applications. Secondly, spatio-temporal correlations may exist due to the effects of dynamic unmeasured covariates and/or biological processes driving the true distribution of the species under study to change across space and/or time \citep{pacifici2017integrating, yuan2017point}. We adjust for these autocorrelations directly in our analysis.  

%Three common questions remain largely unanswered in the literature and providing answers is a focus of this paper. The first question is how one should incorporate observer effort into the analysis of a presence-only dataset, if the observer effort is either known or estimable. The second question is how one should account for potential autocorrelation between sightings due to either repeated sightings of the same individual in quick succession (possibly by different observers), or due to observers sharing knowledge of an individual's location. A failure to remove autocorrelation between sightings or dependence between observers may lead to a biased estimate of true intensity (cite McDonald et al 2013), unless this autocorrelation is appropriately modeled and marginalised out (cite Johnson et al 2013). The third and final question is how one should account for residual spatio-temporal correlations due to the effects of unmeasured covariates and/or biological processes driving the true distribution of the species under study. We provide a detailed discussion on all three points, with the proposed general framework specifically providing solutions for questions 1 and 3.

%Methods have been developed for accounting for residual spatial correlations in the underlying species' intensity between fixed site locations (cite Pacifici et al 2017 and Yuan Blue Whales paper). This autocorrelation could be due to the effects of unmeasured covariates and/or biological processes driving the true intensity. Furthermore, robust models for reducing the influence of very noisy datasets on inference (cite Pacifici et al 2017) and methods for including low quality data as a covariate in a high quality data model have also been considered as promising options (cite Hanks et al 2011 Pacifici et al 2017). Finally, (spatio-temporal) IPPs have also been considered as the unifying model for estimating resource selection functions (cite McDonald et al 2013 and McDonald et al 2013 2), and this includes when the data are of telemetry type (cite Johnson et al 2013). Two fantastic overviews of the IPP methodologies described above can be found (cite Miller et al 2019 and Hefley et al 2016 ). 

%Following similar lines, the spatial epidemiology community previously developed methods for adjusting for spatially-varying population densities and/or population-at-risk densities when estimating spatio-temporal disease intensity surfaces. One such method, the raised incidence spatial point process model (cite Diggle 1990), again assumes a multiplicative decomposition of the observed intensity surface into a term representing natural spatial variation (e.g. population density) and a term reflecting the local raised incidence (called the raised incidence surface). Unlike the detection probability surface, the natural variation surface is not constrained to lie between 0 and 1. Note that here it is the raised incidence surface that is typically of primary interest. 

%The general framework presented here adapts ideas from the spatial epidemiology literature for ecological applications to successfully adjust for a known or estimable observer effort. Methods developed there for adjusting for spatially-varying population densities and/or population-at-risk densities when estimating spatio-temporal disease intensity surfaces are reviewed. One such method, the raised incidence spatial point process model (cite Diggle 1990), forms the basis of our approach. We argue that in settings where one can (stochastically) emulate spatio-temporal observer effort, by considering observer effort as a natural variation surface, our framework can be used with multiple data types. Substantial uncertainties may surround estimates of observer effort. Our general framework is able to propagate all uncertainties through to inference and hence through to management decisions. 

%As discussed in (cite Gelfand new paper), presence-absence and presence-only data are incompatible without further assumptions and conditions imposed. We introduce these assumptions and conditions and show how typical datasets may be adapted to meet them. Crucially, this approach requires the strict assumption that doubling the amount of observer effort at a location, doubles the expected number of sightings there. Clearly this assumption may not hold for static species (e.g. trees) and thus a regression adjustment approach through the modeling of a detection probability/bias surface would be more appropriate here. Such an approach is possible under our general framework.

%This raised incidence model assumes a multiplicative decomposition of the observed intensity surface into a term representing natural spatial variation (e.g. population density) and a term reflecting the local raised incidence (called the raised incidence surface). We argue that in settings where one can (stochastically) emulate spatio-temporal observer effort, by considering observer effort as a natural variation surface, our framework can be used with opportunistic presence-absence (P-A) data and survey presence-only (P-O), site occupancy, site count and many other types of data. 


%A strict assumption placed on spatial point processes is the independence between sightings, conditioned on the intensity. Thus a failure to remove any autocorrelation between sightings or dependence between observers may lead to a biased estimate of true intensity (cite McDonald et al 2013), unless this autocorrelation is appropriately modeled (e.g. in the form of a stochastic movement model) and marginalised out (cite Johnson et al 2013). This autocorrelation is especially detrimental for highly mobile species. Fortunately, in many such cases, the locations of the species' presence are unknown at the beginning of a day or sampling period. Consequently, the locations of \textbf{initial sightings} may satisfy the necessary requirements of independence under moderate and often achievable assumptions. Such a case is found in our real-world motivating problem. 

%Finally, whilst emulating/estimating the observer effort may be near-impossible for many of the sources of sightings found in presence--only databases, in many cases estimation may be achievable for a subset of the observer types. For example, databases may contain sightings from industries which repeatedly travel estimable, known or even GPS-recorded routes (e.g. fisheries and ecotour operators). Knowledge used to estimate the routes may have substantial error associated with it. Our general framework is able to account for such error and propagate all uncertainties through to inference and hence through to management decisions. Finally, many of the benefits of the previous methodologies for being able to use regression adjustment for controlling for observer bias are incorporated in our model framework.



%Our proposed modeling framework combines the latest developments in spatio-temporal point processes from the species distribution models with the ideas of the SCR-SE models. We further extend the SCR-SE framework to allow for unknown observer effort to be modeled with a set of covariates or externally estimated. To use spatio-temporal point processes for highly mobile species, we adapt the raised incidence spatial point process model \citep{diggle1990point} from spatial epidemiology. This helps to define a new interpretable intensity surface that becomes the modeling target. Datasets of differing type and data-collection protocol, including combinations of both static and mobile observers can be appropriately combined. We highlight the necessary assumptions required for the unbiased estimation of the intercept in the model. Our framework requires that observer effort can be controlled for. This either requires that a set of sufficiently-informative detectability covariates are available, or requires that observer effort is known or can be emulated. Expert knowledge can also be incorporated into the analysis. Uncertainties regarding the observer effort and expert knowledge can be fully propagated through to resulting inference. Additional spatio-temporal correlations can also be captured through the inclusion of random effects. Implementation is made especially easy using the R package inlabru \citep{R,inlabru}, enabling researchers to adapt this framework for use in their applications.   

